Inactivation Decoding Analysis for LT Codes

We provide two analytical tools to model the inactivation decoding process of LT codes. First, a model is presented which derives the expected number of inactivations occurring in the decoding process of an LT code. This analysis is then extended allowing the derivation of the distribution of the number of inactivations. The accuracy of the method is verified by Monte Carlo simulations. The proposed analysis opens the door to the design of LT codes optimized for inactivation decoding.

==> notation.tex <==
\newcommand{\Amatrix}{\mathbf{A}}
\renewcommand{\Bmatrix}{\mathbf{B}}
\newcommand{\Cmatrix}{\mathbf{C}}
\newcommand{\Dmatrix}{\mathbf{D}}


\renewcommand{\c}{\mathsf{c}}
\renewcommand{\b}{\mathsf{b}}
\renewcommand{\r}{\mathsf{r}}
\newcommand{\n}{\mathsf{n}}



\newcommand{\res}{\mathtt{r}}
\newcommand{\inact}{\mathtt{i}}
\newcommand{\act}{\mathtt{a}}
\newcommand{\actset}{\mathscr{A}}
\newcommand{\rippleset}{\mathscr{R}}
\newcommand{\cloudset}{\mathscr{C}}
\newcommand{\image}{\mathscr{I}}
\newcommand{\comp}{\bar{\mathscr{I}}}

\newcommand{\kres}{K^\mathtt{r}}
\newcommand{\kinact}{K^\mathtt{i}}
\newcommand{\kact}{K^\mathtt{a}}

\newcommand{\x}{\mathtt{x}}




\newcommand{\osymb}{c}

\newcommand{\ripple}[1]{ \msr{R}_{#1}}
\newcommand{\cloud}[1]{\msr{C}_{#1}}

\newcommand{\Ripp}{\mathsf{R}}
\newcommand{\Ru}{\Ripp_u}
\newcommand{\ru}{\mathsf{r}_u}
\newcommand{\Cloud}{\mathsf{C}}
\newcommand{\Cu}{\mathsf{C}_u}

\newcommand{\cu}{\mathsf{c}_u}
\newcommand{\bu}{\mathsf{b}_u}
\newcommand{\Nu}{\mathsf{N}_u}
\renewcommand{\nu}{\mathsf{n}_u}
%\renewcommand{\ni}{\mathsf{n}_i}
\renewcommand{\ni}{\mathsf{Q}}

\renewcommand{\S}[1]{\mathsf{S}_{#1}}
\newcommand{\C}[1]{\mathsf{C}_{#1}}
\newcommand{\R}[1]{\Ripp_{#1}}
\newcommand{\N}[1]{\mathsf{N}_{#1}}

\newcommand{\Brv}{\mathsf{B}}
\newcommand{\Erv}{\mathsf{A}}
\newcommand{\erv}{\mathsf{a}}

%\newcommand{\Arv}{\mathsf{A}}
%\newcommand{\arv}{\mathsf{a}}

\newcommand{\Y}{\mathsf{N}}
\newcommand{\y}{\mathsf{n}}

\newcommand{\dmax}{ d_{\max}}

\renewcommand{\deg}{\mathrm{deg}}

%\newcommand{\Ninact }{ N_{\mathrm{inact}}}
\newcommand{\Ninact }{\mathbb{E}[\Y]}
%\newcommand{\fett}[1]{{\bf #1}}

\newcommand{\nb}[1]{\mathcal{N}\left(#1\right)}
\newcommand{\sz}[1]{\left|#1\right|}

\newcommand{\myop}[1]{%
  \mathchoice{\raisebox{8pt}{$\displaystyle #1$}}
             {\raisebox{8pt}{$#1$}}
             {\raisebox{4pt}{$\scriptstyle #1$}}
             {\raisebox{1.6pt}{$\scriptscriptstyle #1$}}}

\newtheorem{mydef}{Definition}
\newtheorem{example}{Example}
\newtheorem{prop}{Proposition}
\newtheorem{algo}{Algorithm}

